PointSplit: Towards On-device 3D Object Detection with Heterogeneous Low-power Accelerators

Running deep learning models on resource-constrained edge devices has drawn significant attention due to its fast response, privacy preservation, and robust operation regardless of Internet connectivity. While these devices already cope with various intelligent tasks, the latest edge devices that are equipped with multiple types of low-power accelerators (i.e., both mobile GPU and NPU) can bring another opportunity; a task that used to be too heavy for an edge device in the single-accelerator world might become viable in the upcoming heterogeneous-accelerator world.To realize the potential in the context of 3D object detection, we identify several technical challenges and propose PointSplit, a novel 3D object detection framework for multi-accelerator edge devices that addresses the problems. Specifically, our PointSplit design includes (1) 2D semantics-aware biased point sampling, (2) parallelized 3D feature extraction, and (3) role-based group-wise quantization. We implement PointSplit on TensorFlow Lite and evaluate it on a customized hardware platform comprising both mobile GPU and EdgeTPU. Experimental results on representative RGB-D datasets, SUN RGB-D and Scannet V2, demonstrate that PointSplit on a multi-accelerator device is 24.7 times faster with similar accuracy compared to the full-precision, 2D-3D fusion-based 3D detector on a GPU-only device.

==> eq/inverse_DWAvg.tex <==
\begin{equation}
    \label{eqn:inverseDWAvg}
    \begin{split}
    f^{(j)} = \frac{\sum_{i=1}^{k} w_i(x)f^{(j)}_i}{\sum_{i=1}^{k} w_i(x)}, 
    \text{ where } w_i(x)= \frac{1}{d(x,x_i)^p}, j=1,...,C
    \end{split}
\end{equation}

==> tab/accuracy_50.tex <==
\begin{table}[t]
\centering
  \caption{\rev{mAP at IoU threshold of 0.5 of VoteNet-based 3D object detectors on SUN RGB-D and Scannet V2 datasets.}}
  \label{tab:pipeline}
  \vspace{-3ex}
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{Precision} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Dataset}\\ 
&   &   SUN RGB-D  & Scannet V2  \\ \midrule
\multirow{3}{*}{FP32} & VoteNet & 31.1 & 30.4 \\
                      & PointPainting & \textbf{32.8} & 31.7 \\
                      & \proposal & 32.7 & \textbf{32.4} \\ 
\hline
{INT8} & \proposal & 32.5 & 30.3 \\     
\bottomrule
\end{tabular}
\vspace{-2ex}
\end{table}

==> tab/baseline.tex <==
% \begin{table}
% \centering
%   \caption{Evaluation results of 2-way SA, and latency }
%   \label{tab:baseline}
%   \begin{tabular}{lcc}
%     \toprule
%     Item & mAP & Latency\\
%     \midrule
%     VoteNet & 56.9 & 5130 \\
%     VoteNet + Pointpainting & 60.2 & 15842 \\
%   \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[t]
\vspace{-3ex}
\centering
  \caption{\textbf{Baseline results.} We use VoteNet with PointPainting as our baseline. mAP is meausred at IoU threshold of 0.25.}
  \label{tab:baseline}
 \resizebox{.9\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{cccrcr}
\toprule
\multirow{2}{*}{Model}  & \multirow{2}{*}{Processors} & \multicolumn{2}{c}{SUN RGB-D}         & \multicolumn{2}{c}{Scannet V2(3 RGB views)}  \\
                        &                             & mAP  & Latency(ms)                    & mAP  & Latency(ms) \\ \midrule
\multirow{2}{*}{VoteNet}        & GPU only                  & 56.9 & 1290 \pm 39              & 54.9 & 4925  \pm 548        \\
                                & GPU + EdgeTPU             & 55.5 & 740  \pm 35              & 54.2 & 1029  \pm 264        \\\hline
\multirow{2}{*}{VoteNet + PointPainting}    & GPU only      & 60.2 & 8259 \pm 76              & 56.4 & 27005 \pm 2008       \\
                                            & GPU + EdgeTPU & 58.7 & 1005 \pm 25              & 55.3 & 2220 \pm 200         \\
                            \bottomrule
\end{tabular}
 } % \resizebox
\vspace{-2ex}
\end{table}




==> tab/bfps_weight.tex <==
\begin{table}[h]
% \vspace{-4ex}
\centering
  \caption{\textcolor{blue}{\textbf{Validation accuracy of different weights given on biased FPS on SUN RGB-D.} AS the weight given to biased FPS increases, mAP improves up to the point when the weight is 2. Because the point set becomes too biased, the weight greater than 2 deteriorates the accuracy.}}
  \label{tab:bfps_weights}

  \begin{tabular}{cc}
    \toprule    
    \textcolor{blue}{Weight} & \textcolor{blue}{mAP} \\
    \midrule
    \textcolor{blue}{0.5} & \textcolor{blue}{60.3} \\
    \textcolor{blue}{1.0} & \textcolor{blue}{60.4} \\
    \textcolor{blue}{1.5} & \textcolor{blue}{61.3} \\
    \textcolor{blue}{2.0} & \textcolor{blue}{61.4} \\
    \textcolor{blue}{2.5} & \textcolor{blue}{59.6} \\
    \textcolor{blue}{3.0} & \textcolor{blue}{59.4} \\
  \bottomrule

    \end{tabular}
\vspace{-2ex}
\end{table}

==> tab/eval_result_effect_change.tex <==
\begin{table}
\centering
  \caption{Effect of each change on mAP}
  \label{tab:evalResults_change}
  \begin{tabular}{lc}
    \toprule
    Item & mAP\\
    \midrule
    Baseline & 54.9 \\
    + Quantization-friendly structure & 56.0 \\
    + Pointpainting & 58.8 \\
    + 2-way set abstraction layer & 59.2 \\
    + Quantization & 56.1 \\
  \bottomrule
\end{tabular}
\end{table}

==> tab/eval_scannet_class_25.tex <==
\begin{table*}[t]
\centering
  \caption{Evaluation results on Scannet V2 validation dataset at IoU threshold 0.25.}
  \label{tab:evalScannetClass_25}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
  \begin{tabular}{ccccccccccccccccccccc}
    \toprule
     & Cab & Bed & Chair & Sofa & Table & Door & Wind & Bkshf & Pic & Cntr & Desk & Curt & Fridg & Showr & Toil & Sink & Bath & Gbg & \vline  & Overall\\
    \midrule
    VoteNet                 & 29.8 & 88.6 & 85.4 & 87.7 & 53.2 & 38.1 & 35.4 & 48.1 & 2.6 & 49.9 & 64.6 & 40.4 & 46.3 & 62.7 & 94.7 & 44.0 & 85.9 & 30.9 & \vline & 54.9  \\
    PointPainting & 34.6 & 86.8 & 87.5 & 85.0 & 60.5 & 40.7 & 36.1 & 48.4 & 5.0 & 51.3 & 62.0 & 40.4 & 48.9 & 60.4 & 99.0 & 48.8 & 87.6 & 32.0 & \vline & 56.4 \\
    \proposal (FP32)              & 33.4 & 86.5 & 86.9 & 86.4 & 59.5 & 40.0 & 33.2 & 46.4 & 4.6 & 54.3 & 69.4 & 41.0 & 42.5 & 59.8 & 96.5 & 50.5 & 86.3 & 32.6 & \vline & 56.1 \\
    \proposal (INT8)   & 34.5 & 87.5 & 87.0 & 85.3 & 58.9 & 40.6 & 33.6 & 46.1 & 4.7 & 49.4 & 67.2 & 41.9 & 46.3 & 55.5 & 96.2 & 47.4 & 84.9 & 30.9 & \vline & 55.4 \\
  \bottomrule

    \end{tabular}
} % \resizebox
\end{table*}

==> tab/eval_scannet_class_50.tex <==
\begin{table*}[t]
\vspace{-4ex}
\centering
  \caption{Evaluation results on Scannet V2 validation dataset at IoU threshold 0.5.}
  \label{tab:evalScannetClass_50}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
  \begin{tabular}{ccccccccccccccccccccc}
    \toprule
    Item                    & Cab  & Bed  & Chair & Sofa & Table & Door & Wind & Bkshf & Pic & Cntr & Desk & Curt & Fridg & Showr & Toil & Sink & Bath & Gbg & \vline  & Overall\\
    \midrule
    Votenet                 &  4.6 & 77.0 & 61.3  & 65.7 & 36.9  &  9.8 &  8.9 & 33.8  & 0.0 & 3.0  & 29.4 & 13.7 & 24.1  &  5.7  & 81.4 & 21.3 & 63.7 & 7.0 & \vline & 30.4  \\
    Votenet + PointPainting &  7.1 & 75.9 & 63.8  & 63.9 & 41.3  & 12.7 &  8.3 & 38.4  & 0.3 & 11.4 & 30.6 & 14.9 & 34.0  &  4.4  & 69.0 & 15.2 & 70.5 & 9.3 & \vline & 31.7  \\
    \proposal               &  6.0 & 72.6 & 61.1  & 67.4 & 40.5  & 10.3 &  9.8 & 32.6  & 0.5 & 21.4 & 41.6 & 15.3 & 21.2  &  10.5 & 76.8 & 16.0 & 71.8 & 8.1 & \vline & 32.4  \\
    \proposal - Quantized   &  7.1 & 72.7 & 58.8  & 63.2 & 41.0  & 12.1 &  9.7 & 27.5  & 0.5 & 21.4 & 36.0 & 14.5 & 15.6  & 6.6  & 76.1 & 13.5 & 61.6 & 7.5 & \vline & 30.3  \\
  \bottomrule

    \end{tabular}
} % \resizebox
% \vspace{-4ex}
\end{table*}

==> tab/eval_sunrgbd_class_50.tex <==
\begin{table*}[t]
\centering
  \caption{Evaluation results on SUN RGB-D validation dataset at IoU threshold 0.5.}
  \label{tab:evalSunrgbdClass_50}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line

  \begin{tabular}{ccccccccccccc}
    \toprule
    Item & Bathtub & Bed & Bookshelf & Chair & Desk & Dresser & Nightstand & Sofa & Table & Toilet & \vline & Overall\\
    \midrule
    Votenet                 & 41.3 & 50.5 &  3.8 & 49.8 &  4.4 & 13.3 & 28.1 & 43.2 & 18.0 & 58.6 & \vline & 31.1 \\
    Votenet + PointPainting & 28.0 & 55.8 &  7.3 & 48.2 &  4.3 & 19.0 & 29.4 & 57.1 & 18.4 & 60.4 & \vline & 32.8 \\
    \proposal               & 18.3 & 51.8 &  9.3 & 49.2 &  5.8 & 21.9 & 28.5 & 59.2 & 21.9 & 61.2 & \vline & 32.7 \\
    \proposal - Quantized   & 29.9 & 53.2 &  6.8 & 47.2 &  5.7 & 19.1 & 28.5 & 55.6 & 20.5 & 58.7 & \vline & 32.5 \\
  \bottomrule

    \end{tabular}
} % \resizebox

\end{table*}

==> tab/inference_time.tex <==
\begin{table}
\centering
  \caption{Inference time measured on Jetson Nano}
  \label{tab:inferenceTime}
  \begin{tabular}{ccc}
    \toprule
    Model & Processors & Inference time (in ms)\\
    \midrule
    \multirow{2}{*}{Baseline(VoteNet)} & GPU Only & 5130  \\
                                   & GPU + EdgeTPU & 931 \\
    \multirow{2}{*}{VoteNet + PointPainting} & GPU Only & 15842  \\
                                   & GPU + EdgeTPU & 1214 \\
    LuxMea & GPU + EdgePTU & 1206 \\
    LuxMea(Pieplined) & GPU + EdgePTU & 854 \\
  \bottomrule
\end{tabular}
\end{table}

==> tab/pipeline2.tex <==
% \begin{table}[]
% \centering
%   \caption{Evaluation results of 2-way SA, and latency }
%   \label{tab:pipeline}
% \begin{tabular}{@{}llll@{}}
% \toprule
% Processors                 & Item                    & mAP  & Latency \\ \midrule
% GPU Only                   & Votenet + Pointpainting & 60.2 & 15842   \\
% \multirow{2}{*}{GPU + TPU} & 2-way SA                & 61.8 & 1206    \\
%                           & Pipelining              & 61.8 & 854     \\ \cmidrule(l){1-4} 
% \end{tabular}
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
  \caption{\textbf{Evaluation results and latency.} Latency is reduced to 759ms and 1444ms for \proposal pipelined while keeping mAP at 59.9 and 55.7 on SUN RGB-D and Scannet V2 dataset. mAP is meausred at IoU threshold of 0.25.}
  \label{tab:pipeline}
%\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Processors} & \multirow{2}{*}{Method}   & \multirow{2}{*}{Quantization} & \multicolumn{2}{c}{SUN RGB-D (primary)}      & \multicolumn{2}{c}{Scannet V2 (secondary)}                           \\ 
    &   &   & mAP  & \multicolumn{1}{c}{Latency(ms)} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Latency(ms)} \\ \midrule
\multirow{4}{*}{GPU only}                   & No fusion                 & FP32  & 56.9 & 1290 \pm 39  & 54.9  & 4925 \pm 548     \\
                                            &  PointPainting & FP32  & 60.2 & 8259 \pm 76  & \textbf{56.4}  & 27005 \pm 2008     \\
                                            & Random split            & FP32  & 60.4   & 8229 \pm 94 & 55.2  &  26157 \pm 2030     \\ 
                                            & \proposal w/o pipelining               & FP32  & \textbf{61.4} & 8188 \pm 25 & 56.1  &  26848 \pm 417      \\ \hline
\multirow{4}{*}{GPU + EdgeTPU}              & No fusion               & INT8 & 55.5 & 740 \pm 35  & 54.2  & 1029 \pm 264   \\     
                                            & PointPainting & INT8 & 58.7 & 1005 \pm 25  & 55.3  & 2220 \pm 200      \\
                                         & \proposal w/o pipelining              & INT8 & \textbf{59.9} & 991 \pm 23  & \textbf{55.7}  & 1887 \pm 253      \\
                                            & \proposal   & INT8 & \textbf{59.9} & 759 \pm 14   & \textbf{55.7}  & 1444 \pm 177       \\ \bottomrule
\end{tabular}
%} 
\end{table*}
